A New Distribution-Free Concept for Representing, Comparing, and Propagating Uncertainty in Dynamical Systems with Kernel Probabilistic Programming

This work presents the concept of kernel mean embedding and kernel probabilistic programming in the context of stochastic systems. We propose formulations to represent, compare, and propagate uncertainties for fairly general stochastic dynamics in a distribution-free manner. The new tools enjoy sound theory rooted in functional analysis and wide applicability as demonstrated in distinct numerical examples. The implication of this new concept is a new mode of thinking about the statistical nature of uncertainty in dynamical systems.

==> arxiv 2/jzpreamble.tex <==
% ========================================================================
% jz preambles
% ========================================================================

% theorems and proofs
\usepackage{amsmath}

\usepackage{amssymb}
\usepackage{algorithm}
\usepackage{algorithmic}

% \theoremstyle{plain}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{definition}{Definition}[section]
\newtheorem{proposition}{Proposition}[section]
\newtheorem{lemma}{Lemma}[section]
\newtheorem{statement}{Statement}[section]
\newtheorem{question}{Question}[section]
\usepackage{graphicx}

% use amsthm
% \usepackage{amsthm}
% \let\proof\relax
% \let\endproof\relax


% \usepackage{wrapfig}

% \theoremstyle{remark}
% \newtheorem{remark}{Remark}

% \theoremstyle{definition}
% \newtheorem{definition}{Definition}[section]

% ----------------------------------------------
% %  margin type 1. old
\usepackage{xcolor,soul}
% \usepackage[heightrounded,marginparwidth=2.5cm,marginparsep=3mm]{geometry}
% \usepackage{marginnote}

% % for margin comments
% % \newcommand{\jz}[1]{\marginpar{\Tiny\color{blue}{#1}}}
% \newcommand{\jz}[1]{\marginnote{\small\hl{#1}}}

% % inline notes
% \newcommand{\jz}[1]{ {\color{red} {\small\hl{#1}}} }
% \newcommand{\km}[1]{ {\color{blue} {\small\hl{#1}}} }
% \newcommand{\todo}[1]{ {\color{blue} todo {\small\hl{#1}} } }

% use the following to turn off comments
% \newcommand{\jz}[1]{}

% margin type 2
% another type of todo list
% \usepackage[heightrounded,marginparwidth=2.5cm,marginparsep=3mm]{geometry}
% \usepackage[colorlinks]{hyperref}
% \usepackage[colorinlistoftodos]{todonotes}
% \newcommand{\jz}[1]{\todo[color=yellow]{#1}}
% \usepackage{xspace
% }
% \setlength{\marginparwidth}{3.5cm}
% ----------------------------------------------

% for 


%used for term/notation for hmpc
% \newcommand{\thisalg}{LNMS\xspace}
% \newcommand{\moseq}{\ensuremath{\mathcal{M}}\xspace}
% \newcommand{\feasr}{\ensuremath{\mathcal{X}^{\mathcal{M}}}\xspace} % feasible region

% % ifac kpp paper kme paper
% % collocation nodes
% \usepackage{xspace}
\newcommand{\colnode}{\ensuremath{\{\xi ^1, \xi ^2, \dots, \xi ^N\} }}
\usepackage{savesym}
\savesymbol{AND}
% \usepackage{subcaption} % figures side by side
% \usepackage{subfig}
% ========================================================================

